PsycheMME: A Psychology-Informed Benchmark for Social Understanding and Interaction in Videos

Understanding human needs and selecting responses require distinct judgments that aggregate accuracy can obscure. We introduce PsycheMME, a video benchmark informed by psychology, with eight capabilities spanning grounding, states, needs, interaction decisions, memory, and risk. Drawing on Social Information Processing and the Perception-Action Cycle, this organization separates human understanding from response selection. We construct 1,000 questions from 630 episodes through independent answering with proposed references withheld and expert review. Our Reasoning-Verified protocol weights answer credit by the support and logical consistency of explicit rationales against annotated cues. Across 17 models, Timing has the lowest Verified scores and credit retention, with weaker support judgments for correct Timing answers. Models with similar Need scores still differ in answer completeness on open questions. Input controls and SFT/GRPO examine context dependence and adaptation. Evaluating answers alongside rationales locates where models fail across understanding, response selection, and justification.

==> table/understanding_decisions.tex <==
\begin{table}[H]
\centering
\caption{Exploratory Qwen association on 173 links from 101 episodes. $U$ and $D$ denote correctness of the linked understanding and decision answers. Gap and 95\% CI are in percentage points.}
\label{tab:app_ud}
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\psycheapptablefit{%
\begin{tabular}{lrrrr}
\toprule
Model & \shortstack{$P(D=1)$\\$U=1$} & \shortstack{$P(D=1)$\\$U=0$} & Gap & 95\% CI \\
\midrule
Qwen3.5-9B & 60.13 & 26.67 & 33.46 & [5.80, 56.25] \\
\bottomrule
\end{tabular}}
\end{table}

